CNN-based Dendrite Core Detection from Microscopic Images of Directionally Solidified Ni-base Alloys

Dendrite core is the center point of the dendrite. The information of dendrite core is very helpful for material scientists to analyze the properties of materials. Therefore, detecting the dendrite core is a very important task in the material science field. Meanwhile, because of some special properties of the dendrites, this task is also very challenging. Different from the typical detection problems in the computer vision field, detecting the dendrite core aims to detect a single point location instead of the bounding-box. As a result, the existing regressing bounding-box based detection methods can not work well on this task because the calculated center point location based on the upper-left and lower-right corners of the bounding-box is usually not precise. In this work, we formulate the dendrite core detection problem as a segmentation task and proposed a novel detection method to detect the dendrite core directly. Our whole pipeline contains three steps: Easy Sample Detection (ESD), Hard Sample Detection(HSD), and Hard Sample Refinement (HSR). Specifically, ESD and HSD focus on the easy samples and hard samples of dendrite cores respectively. Both of them employ the same Central Point Detection Network (CPDN) but do not share parameters. To make HSD only focus on the feature of hard samples of dendrite cores, we destroy the structure of the easy samples of dendrites which are detected by ESD and force HSD to learn the feature of hard samples. HSR is a binary classifier which is used to filter out the false positive prediction of HSD. We evaluate our method on the dendrite dataset. Our method outperforms the state-of-the-art baselines on three metrics, i.e., Recall, Precision, and F-score.

==> 0_abstract.tex <==

Dendrite core is the center point of the dendrite. The information of dendrite core is very helpful for material scientists to analyze the properties of materials. Therefore, detecting the dendrite core is a very important task in the material science field. Meanwhile, because of some special properties of the dendrites, this task is also very challenging. Different from the typical detection problems in the computer vision field, detecting the dendrite core aims to detect a single point location instead of the bounding-box. As a result, the existing regressing bounding-box based detection methods can not work well on this task because the calculated center point location based on the upper-left and lower-right corners of the bounding-box is usually not precise. In this work, we formulate the dendrite core detection problem as a segmentation task and proposed a novel detection method to detect the dendrite core directly. Our whole pipeline contains three steps: Easy Sample Detection (ESD), Hard Sample Detection(HSD), and Hard Sample Refinement (HSR). Specifically, ESD and HSD focus on the easy samples and hard samples of dendrite cores respectively. Both of them employ the same Central Point Detection Network (CPDN) but do not share parameters. To make HSD only focus on the feature of hard samples of dendrite cores, we destroy the structure of the easy samples of dendrites which are detected by ESD and force HSD to learn the feature of hard samples. HSR is a binary classifier which is used to filter out the false positive prediction of HSD. We evaluate our method on the dendrite dataset. Our method outperforms the state-of-the-art baselines on three metrics, i.e., Recall, Precision, and F-score.


==> 3_DiscussionMotivation.tex <==
% \chapter{Motivations and Challenges}
% \label{chapter:motivation}

% Intuitively, we can use two networks to detect the center point location of the dendrite. Specifically, using the first networks to detect the dendrite cores in the input image. We denote the dendrites which are detected in the first network easy samples and denote the other dendrites hard samples. Then, using the second network to detect the hard samples. In the end, combining the detected results from these two networks to get the final prediction result. However, using this method can not get the expected result. From the first row in \tableref{tab:crop_size} we can find that this scenario leads to pretty low precision. We show the visualization result of this method in \figref{fig:motivation_1} and observe that training two networks to detect the dendrite cores directly will lead to these two networks learning similar features from the input images. As a result, the second network also intended to detect the easy samples instead of the hard ones. From the \figref{fig:motivation_1} we can see that the dendrites in the yellow boxes are detected by both of these two networks. Therefore, exploiting a novel technique to force these two networks to detect the easy samples and hard samples separately is necessary.

% %------------------------------
% \begin{figure*}
% \centering
% \includegraphics[width=1.0\linewidth]{images/motivation_1.pdf}
% \vspace{-40pt}
% \caption{ Three visualization results of using two networks to detect the dendrite cores directly. The red triangles denote the ground truth, the green triangles denote the dendrite cores detected by the first network, the blue triangles denote the dendrite cores detected by the second network, and the dendrites in the yellow boxes mean these dendrites can be detected by both of these two networks.
% }
% \label{fig:motivation_1}
% \vspace{-10pt}
% \end{figure*}
% %------------------------------

==> 4_copy.tex <==
\chapter{Methodology}


%------------------------------
\begin{figure*}
\centering
\includegraphics[width=1.0\linewidth]{images/new_pipline.pdf}
\vspace{-40pt}
\caption{ The whole pipeline of the Two-stage detection method. ESDN and HSDN are implemented based on \cite{newell2016stacked} and they have the same architecture without sharing the parameter. BCN is implemented based on ResNet-50. The predicted dendrite cores in $\mathbf{O}$ come from $\mathbf{O}_1$ and $\mathbf{O}_2$. The upper points of the red triangles and the lower points of green triangles denote the ground truth and the predicted dendrite cores respectively.
}
\label{fig:pipline}
\vspace{-10pt}
\end{figure*}
%------------------------------


\section{Two-stage detection}

In this work, we formulate the dendrite core detection problem as a segmentation task. In the end, the network predicts a heatmap $\mathbf{H}$ with the size 512*512. The network predicts a dendrite core at the location $\mathbf{a}$ if the value of location $\mathbf{a}$ in the heatmap is equal to one and other locations are taken as background. The whole pipeline contains three components: Easy Samples Detection Network(ESDN), Hard Samples Detection network(HSDN), and Binary Classification Network(BCN). Specifically, first, ESDN detects the easy samples of dendrite cores. Then we destroy the structure of the easy samples of dendrites detected by ESDN from the input image. The cropped images will be used to train HSDN. Because the image input into HSDN only contains hard samples of dendrite cores, the Precision of HSDN is relatively lower than ESDN. To alleviate this problem, we add BCN after HSDN. The input of BCN is only a small patch instead of the whole image, therefore it has the advantage of identifying the true positive samples and false positive samples of dendrite cores detected by HSDN. The whole pipeline is shown in \figref{fig:pipline}. We will elaborate on each component separately in the following paragraphs.

\subsection{Easy Samples Detection Network (ESDN)}
\label{subsec:esdn}

ESDN only focuses on detecting the easy samples of dendrite cores from the input images. We formulate ESDN as \reqref{eq:o1_0}. \begin{align}\label{eq:o1_0}
\mathbf{O}_1 = \mathbf{S}_1(\mathbf{I}_1)
\end{align}
$\mathbf{I}_1$, $\mathbf{S}_1$, and $\mathbf{O}_1$ denote the input image, model, and the predicted heatmap of ESDN respectively. $\mathbf{G}_1$ is the ground truth which is also a heatmap as shown in \figref{fig:gt1_gt2} (d). The architecture of $\mathbf{S}_1$ is similar to \cite{newell2016stacked}. With input $\mathbf{I}_1$ into $\mathbf{S}_1$, it will get the predicted heatmap $\mathbf{O}_1$ as shown in \figref{fig:gt1_gt2} (b). In order to increase the Precision of ESDN, we set up a relatively higher threshold $\alpha$. If the value of $\mathbf{O}_1(i, j)$ in the heatmap is greater than the threshold $\alpha$, we binarize the value of $\mathbf{O}_1(i, j)$ to one, otherwise set the value to zero as shown in \reqref{eq:o1_1}. 
\begin{align}\label{eq:o1_1}
\mathbf{O}_1(i, j)= \left\{\begin{matrix}
 1,~\text{if}~\mathbf{O}_1(i, j) \mathbf{>} \alpha,\\ 
0,\quad \quad \text{otherwise}.
\end{matrix}
\right.
\end{align}
$(i, j)$ is the coordinate.

\begin{figure}[h!]
  \includegraphics[width=1.0\textwidth]{images/gt1_gt2.pdf}
  \centering
  \vspace{-25pt}
 \caption{The illustration of input (a), predicted heatmap (b), ground truth (d) of ESDN and input (c), ground truth (e) of HSDN.}
  \label{fig:gt1_gt2}
\end{figure}



\subsection{Hard Samples Detection Network (HSDN)}
\label{subsec:hsdn}

HSDN is designed to focus on the hard samples of dendrite cores in the input images. HSDN and ESDN have the same architecture without sharing the parameter. As discussed in \secref{chapter:motivation}, if we input $\mathbf{I}_1$ into HSDN directly without any processing, it will make both ESDN and HSDN learn the similar features from the input image. As a result, HSDN will not learn the features from the hard samples of dendrites. To solve this problem, in this work, we propose to destroy the structure of the easy samples of dendrites that are detected by ESDN. Specifically, we crop out the easy samples of dendrites from $\mathbf{I}_1$ and denote the image after such cropping to be $\mathbf{I}_2$ as shown in \figref{fig:gt1_gt2} (c). 

$\mathbf{I}_2$ is the input of HSDN. In addition to destroying the structure of easy samples of dendrites, it also needs to generate the ground truth $\mathbf{G}_2$ which is a heatmap as shown in \figref{fig:gt1_gt2} (e) for training HSDN. The ground truth $\mathbf{G}_2$ can be gotten from \reqref{eq:g2}. 
\begin{align}\label{eq:g2}
\mathbf{G}_2(i, j)= \left\{\begin{matrix}
\quad\mathbf{0}, \quad \quad \quad \quad   ~\text{if}~\mathbf{O}_1(i, j) \mathbf{=} \mathbf{1},\\ 
\mathbf{G}_1(i, j),\quad \quad \quad \quad \text{otherwise}.
\end{matrix}
\right.
\end{align}
Then we can train the HSDN with the input image $\mathbf{I}_2$ and ground truth $\mathbf{G}_2$. $\mathbf{O}_2$ is the predicted heatmap of HSDN as shown in \reqref{eq:o2_0}.  
\begin{align}\label{eq:o2_0}
\mathbf{O}_2 = \mathbf{S}_2(\mathbf{I}_2)
\end{align}
$\mathbf{S}_2$ is the model of HSDN. Different from ESDN, we set up a relatively lower threshold $\beta$ for $\mathbf{O}_2$ as shown in \reqref{eq:o2_1} 
\begin{align}\label{eq:o2_1}
\mathbf{O}_2(i, j)= \left\{\begin{matrix}
1,~\text{if}~\mathbf{O}_2(i, j) \mathbf{>} \beta,\\ 
0,\quad \quad \text{otherwise}.
\end{matrix}
\right.
\end{align}
because we expect HSDN to detect more hard samples of dendrite cores to increase the recall. The false positive detection will be filtered out by BCN later. In the end, we combine the prediction $\mathbf{O}_1$ from ESDN and $\mathbf{O}_2$ from HSDN together with \reqref{eq:o}.
\begin{align}\label{eq:o}
\mathbf{O}(i, j)= \left\{\begin{matrix}
1,~\text{if}~\mathbf{O}_1(i, j) \mathbf{=} \mathbf{1} ~\text{or}~ \mathbf{O}_2(i, j) \mathbf{=} \mathbf{1},\\ 
0,\quad \quad \quad \quad  \quad \quad  \quad \quad  \text{otherwise}.
\end{matrix}
\right.
\end{align}
$\mathbf{O}$ is the final predicted result. There are many different ways to destroy the structure of the easy samples of dendrites. The crop size and intensity have a big effect on the predicted result. We will exploit the crop size and crop intensity in \secref{subsec:crop} and \secref{subsec:intensity} separately.

%---------------------------------------------------------BCN
\subsection{Binary Classification Network(BCN)}
\label{subsec:bcn}

In order to detect more hard samples of dendrite cores, we use a relatively lower threshold $\beta$ for the $\mathbf{O}_2$ which will lead to a lower Precision for HSDN. To prevent the decrease in Precision, in this work, we add BCN to filter out the false positive samples of dendrite cores detected by HSDN. The BCN is a binary classification model implemented based on the ResNet-50 backbone. The input of BCN is a small patch with the size 80*80. The effectiveness of BCN will be discussed later in \secref{chapter:ablation}.

\textbf{Building the training dataset for BCN.} We randomly crop the 80*80 patches from the original images to build the training dataset for BCN. Specifically, around each dendrite core in the original images, we crop five positive samples and ten negative samples of dendrites. For the positive samples, first we draw a circle $\mathbf{A}$ as shown in \figref{fig:bcn_sample} around each of dendrite cores with the radius 4 pixels. Then we randomly choose five locations inside circle $\mathbf{A}$ and crop a patch with the size 80*80 around each of the five locations. It is the same for the negative samples, we draw another two circles $\mathbf{B}$, $\mathbf{C}$ as shown in \figref{fig:bcn_sample} around each of dendrite cores with the radius 15 and 40 pixels respectively. Then we randomly choose five locations inside the green area of circle $\mathbf{B}$, blue area of circle $\mathbf{C}$ respectively and crop a patch with the size 80*80 around each of the locations. We show a positive sample in \figref{fig:bcn_sample} (b) and two negative samples in \figref{fig:bcn_sample} (c), (d).

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.8\textwidth]{images/BCN_samples.pdf}
  \vspace{-25pt}
  \caption{Building the training set for BCN. The positive samples are cropped around the randomly selected points inside circle $\mathbf{A}$, the negative samples are cropped around the randomly selected points inside the green area of circle $\mathbf{B}$ and the blue area of circle $\mathbf{C}$. The circles $\mathbf{A}$, $\mathbf{B}$, and $\mathbf{C}$ are around the dendrite core with radius 4, 15, 40 pixels respectively. (b) is an example of the positive sample and (c), (d) are the examples for negative samples.}
  \label{fig:bcn_sample}
\end{figure}

%---------------------------------------------------------
	
%---------------------------------------------------------loss function	
\subsection{Loss function}
We follow the previous work in \cite{newell2016stacked} and use $\mathbf{L}_2$ loss to optimize the network. ESDN and HSDN use the same loss function as shown in \reqref{eq:loss}. 
\begin{align}\label{eq:loss}
\mathcal{L}(\mathbf{I}, \mathbf{G}) ~\text{=}~ \lambda * \mathbf{L}_2(\mathbf{I}, \mathbf{G})
\end{align}
$\mathbf{I}$ and $\mathbf{G}$ are the corresponding input and ground truth for ESDN and HSDN respectively.
%---------------------------------------------------------

%--------------------------------------------------------- Exploit the Crop size
\section{Exploit the crop size}
\label{subsec:crop}

\begin{figure}[h!]
  \includegraphics[width=1\textwidth]{images/crop_sample.pdf}
  \vspace{-25pt}
  \caption{The visualization of different crop sizes. (a) denotes the crop size 40*40, (b) denotes the crop size 60*60, (c) denotes the crop size 80*80, and (d) denotes the crop size 100*100.}
  \label{fig:crop_size}
\end{figure}

During the procedure of destroying the structure of easy samples of dendrites detected by ESDN, the crop size is a big fact that can affect the final detected result. In order to exploit the reasonable crop size, we have conducted a series of experiments. We take different crop sizes to destroy the structure of easy samples of dendrites. Specifically, we use the crop size 40*40, 60*60, 80*80, 100*100, and no crop. The visualization results of the cropped images are displayed in \figref{fig:crop_size}. 

We evaluate the Recall, Precision, and F-score with different crop sizes and show the results in \tableref{tab:crop_size} and \figref{fig:crop_curve}. From \figref{fig:crop_curve}, we can see that \ding{182} Without destroying the structure of easy samples of dendrites detected by ESDN, the final F-score is very low. \ding{183} It reaches the best F-score when the crop size is 80*80. When continue to increase the crop size to 100*100, the F-score begins to decrease. The reason for this result is that the smaller crop size or without cropping can not destroy the structure of dendrites detected by ESDN and the larger crop size may destroy the potential dendrites which should be detected by HSDN. Based on these observations, we finally choose the crop size 80*80.

\begin{figure}[h!]
  \includegraphics[width=1\textwidth]{images/crop_curve.pdf}
  \vspace{-25pt}
  \caption{Exploiting the optimal crop size. Red points denote the Recall, green points denote the Precision, and blue points denote the F-score. When the crop size is equal to 80*80, it gets the best F-score.}
  \label{fig:crop_curve}
\end{figure}

%----------crop_size----------------
\begin{table*}
\centering
\small
{
    \resizebox{0.8\linewidth}{!}{
    {
	\begin{tabular}{l|c|c|c}
		
    \toprule
     \multicolumn{1}{l|}{Crop size} & \multicolumn{1}{c|}{Recall$\uparrow$} & \multicolumn{1}{c|}{Precision$\uparrow$}  & \multicolumn{1}{c}{F-Score$\uparrow$}  \\
     
   \midrule
                 
       no crop  & 0.9633 & 0.8229 & 0.8876\\
   
   \midrule
                
       40*40  & 0.9628 & 0.9546 & 0.9587\\
 
    \midrule
                
       60*60  & 0.9675 & 0.9544 & 0.9609\\

    \midrule
  
      \topone{80*80}  & \topone{0.9670} & \topone{0.9563} & \topone{0.9616}\\

    \midrule
              
       100*100  & 0.9654 & 0.9523 & 0.9588\\

    \bottomrule
		
	\end{tabular}
	}
	}
}
\vspace{-15pt}
\caption{Exploiting the optimal crop size when the deviation distance is 10 pixels. In this work, we try the crop size: 40*40, 60*60, 80*80, 100*100, and no crop.}
\label{tab:crop_size}
\end{table*}

%---------------------------


%---------------------------------------------------------

%--------------------------------------------------------- Exploit the intensity
\section{Exploit the intensity}
\label{subsec:intensity}

\subsection{Fill the cropped area with fixed intensity}
\label{subsec:intensity_fixe}

In addition to the crop size, the crop intensity also has a big influence on the prediction result of HSDN. In this work, we conduct a series of experiments to exploit the optimal crop intensity. Specifically, we use the fixed intensities 0, 128, and 255. Based on the discussion in \secref{subsec:crop}, using crop size 80*80 can reach the best F-score. Therefore, we only consider the crop size 80*80 here. The visualization results of different crop intensity are shown in \figref{fig:crop_intensity}. We also evaluate the Recall, Precision, and F-score with the different intensities. From \figref{fig:intensity_curve} we find that with the intensity 0, it can get the best F-score. Finally, we choose the intensity 0 in this work.

\begin{figure}[h!]
  \includegraphics[width=1\textwidth]{images/intensity_sample.pdf}
  \vspace{-25pt}
  \caption{Exploiting the optimal intensity to fill the cropped area. The intensity in the cropped areas is 0 for (a), 255 for (b), and 128 for (c).}
  \label{fig:crop_intensity}
\end{figure}

\begin{figure}[h!]
  \includegraphics[width=1\textwidth]{images/intensity_curve.pdf}
  \vspace{-25pt}
\caption{Exploiting the optimal intensity to fill the cropped area. In this work, we trial three intensities 0, 128, and 255. Red points denote the Recall, green points denote the Precision, and blue points denote the F-score. When the intensity is equal to 0, it gets the best F-score.}
  \label{fig:intensity_curve}
\end{figure}

\subsection{Process the cropped area with Gaussian blur}

In addition to filling the cropped area with the fixed intensity, we also exploit using the Gaussian blur to process the cropped area. Based on the discussion in \secref{subsec:intensity_fixe}, using the intensity 0, the HSDN can get the best F-score. Therefore, we use the Gaussian blur to process the edges of the cropped areas with intensity 0. The visualization results are shown in \figref{fig:gaussian_sample} (a). Besides, we have a trial to process the cropped areas only with Gaussian blur. The visualization results are shown in \figref{fig:gaussian_sample} (b). From \tableref{tab:intensity} we can see that with the fixed intensity 0, it can get the best F-score.

\begin{figure}[h!]
  \includegraphics[width=1\textwidth]{images/gaussian_sample.pdf}
  \vspace{-25pt}
\caption{Using Gaussian blur to process cropped areas. (a) denotes first to fill the cropped area with intensity 0 and then use Gaussian blur to process the edges. (b) denotes process the cropped areas by Gaussian blur directly.}
  \label{fig:gaussian_sample}
\end{figure}

%-----------intensity----------------
\begin{table*}
\centering
\small
{
    \resizebox{0.8\linewidth}{!}{
    {
	\begin{tabular}{l|c|c|c}
		
    \toprule
      \multicolumn{1}{l|}{intensity} & \multicolumn{1}{c|}{Recall$\uparrow$} & \multicolumn{1}{c|}{Precision$\uparrow$}  & \multicolumn{1}{c}{F-Score$\uparrow$}  \\
    
    \midrule
 
      \topone{0}  & \topone{0.9670} & \topone{0.9563} & \topone{0.9616}\\
   
   \midrule
             
       128  & 0.9659 & 0.9478 & 0.9568\\

    \midrule
             
       255  & 0.9675 & 0.9549 & 0.9612\\

   \midrule
             
       Gaussian & 0.9617 & 0.9597 & 0.9607\\ 

    \midrule
            
       0 + Gaussian  & 0.9617 & 0.9541 & 0.9579\\

    \bottomrule
		
	\end{tabular}
	}
	}
}
\vspace{-15pt}
\caption{Exploiting the optimal intensity in the cropped areas when deviation distance is 10 pixels and cropped size is 80*80. 0 + Gaussian means first filling the cropped areas with intensity 0 and then processing the edges by Gaussian blur.}
\label{tab:intensity}
\end{table*}
%---------------------------


%---------------------------------------------------------

%--------------------------------------------------------- Training detail
\section{Training detail}

We first train ESDN with a learning rate of 0.0004.  Then, we train HSDN with a learning rate of 0.0001 by fixing the parameter of ESDN. We train both ESDN and HSDN 100 epochs. Finally, we train BCN 50 epochs with a learning rate of 0.0001. We set up the threshold $\alpha$ in ESDN to 0.4,  the threshold $\beta$ in HSDN to 0.1, and $\lambda$ in the loss function to 0.5. The experiments are conducted on the same platform with two NVIDIA Tesla V100 GPUs.

%---------------------------------------------------------











==> precis.tex <==
%-----------comparison----------------
\begin{table*}
\centering
\small
{
    \resizebox{1.0\linewidth}{!}{
    {
	\begin{tabular}{l|l|c|c|c}
		
    \toprule
     \multicolumn{1}{l|}{Methods} & \multicolumn{1}{l|}{deviation} & \multicolumn{1}{c|}{Recall$\uparrow$} & \multicolumn{1}{c|}{Precision$\uparrow$}  & \multicolumn{1}{c}{F-Score$\uparrow$}  \\
   \midrule
   \multirow{2}{*}{SSD}                
      & 10  & 0.9585 & 0.9415 & 0.9499\\
      & 20  & 0.9659 & 0.9488 & 0.9573\\
      
    \midrule
    \multirow{2}{*}{Faster-RCNN}   
    & 10    & 0.9112 & 0.9050 & 0.9081\\
    & 20    & 0.9633 & 0.9567 & 0.9600\\

    \midrule
    \multirow{1}{*}{Stacked-Hourglass}   
     & 10   &  0.9564 & 0.9559 & 0.9561\\
     
    \midrule
    \multirow{1}{*}{\topone{Ours}}   
     & \topone{10}  & \topone{0.9638} & \topone{0.9710} & \topone{0.9674}\\

    \bottomrule
		
	\end{tabular}
	}
	}
}
\caption{Comparison results}
\label{tab:comparison}
%\vspace{-10pt}
\end{table*}
%---------------------------


%-----------ablation----------------
\begin{table*}
\centering
\small
{
    \resizebox{1.0\linewidth}{!}{
    {
	\begin{tabular}{l|l|c|c|c}
		
    \toprule
     \multicolumn{1}{l|}{Methods} & \multicolumn{1}{l|}{deviation} & \multicolumn{1}{c|}{Recall$\uparrow$} & \multicolumn{1}{c|}{Precision$\uparrow$}  & \multicolumn{1}{c}{F-Score$\uparrow$}  \\
   \midrule
   \multirow{1}{*}{One-Stage}                
      & 10  & 0.9341 & 0.9745 & 0.9538\\
      
    \midrule
    \multirow{1}{*}{Two-Stage}   
    & 10    & 0.9670 & 0.9563 & 0.9616\\

    \midrule
    \multirow{1}{*}{\topone{Two-Stage + BC}}   
     & \topone{10}  & \topone{0.9638} & \topone{0.9710} & \topone{0.9674}\\

    \bottomrule
		
	\end{tabular}
	}
	}
}
\caption{Ablation study on one-stage, two-state, and two-stage + binary classification}
\label{tab:ablation}
%\vspace{-10pt}
\end{table*}


%----------crop_size----------------
\begin{table*}
\centering
\small
{
    \resizebox{1.0\linewidth}{!}{
    {
	\begin{tabular}{l|l|c|c|c}
		
    \toprule
     \multicolumn{1}{l|}{Methods} & \multicolumn{1}{l|}{Crop size} & \multicolumn{1}{c|}{Recall$\uparrow$} & \multicolumn{1}{c|}{Precision$\uparrow$}  & \multicolumn{1}{c}{F-Score$\uparrow$}  \\
     
   \midrule
   \multirow{1}{*}{Two-Stage}                
      & no crop  & 0.9633 & 0.8229 & 0.8876\\
   
   \midrule
   \multirow{1}{*}{Two-Stage}                
      & 40 x 40  & 0.9628 & 0.9546 & 0.9587\\
 
    \midrule
   \multirow{1}{*}{Two-Stage}                
      & 60 x 60  & 0.9675 & 0.9544 & 0.9609\\

    \midrule
   \multirow{1}{*}{\topone{Two-Stage}}   
     & \topone{80 x 80}  & \topone{0.9670} & \topone{0.9563} & \topone{0.9616}\\

    \midrule
   \multirow{1}{*}{Two-Stage}                
      & 100 x 100  & 0.9654 & 0.9523 & 0.9588\\

    \bottomrule
		
	\end{tabular}
	}
	}
}
\caption{Exploit influence of cropped size when the deviation distance is 10 pixels}
\label{tab:crop_size}
%\vspace{-10pt}
\end{table*}

%---------------------------


%-----------intensity----------------
\begin{table*}
\centering
\small
{
    \resizebox{1.0\linewidth}{!}{
    {
	\begin{tabular}{l|l|c|c|c}
		
    \toprule
     \multicolumn{1}{l|}{Methods} & \multicolumn{1}{l|}{intensity} & \multicolumn{1}{c|}{Recall$\uparrow$} & \multicolumn{1}{c|}{Precision$\uparrow$}  & \multicolumn{1}{c}{F-Score$\uparrow$}  \\
    
    \midrule
   \multirow{1}{*}{\topone{Two-Stage}}   
     & \topone{0}  & \topone{0.9670} & \topone{0.9563} & \topone{0.9616}\\
   
   \midrule
   \multirow{1}{*}{Two-Stage}                
      & 128  & 0.9659 & 0.9478 & 0.9568\\

    \midrule
   \multirow{1}{*}{Two-Stage}                
      & 255  & 0.9675 & 0.9549 & 0.9612\\

   \midrule
   \multirow{1}{*}{Two-Stage}                
      & Gaussian & 0.9617 & 0.9597 & 0.9607\\ 

    \midrule
   \multirow{1}{*}{Two-Stage}                
      & 0 + Gaussian  & 0.9617 & 0.9541 & 0.9579\\

    \bottomrule
		
	\end{tabular}
	}
	}
}
\caption{Exploit influence of intensity in the cropped area when deviation distance is 10 pixels and cropped size is 80 x 80}
\label{tab:intensity}
%\vspace{-10pt}
\end{table*}
%---------------------------
